Algebraic properties of the first-order part of a problem

In this paper we study the notion of first-order part of a computational problem, first introduced by Dzhafarov, Solomon, and Yokoyama, which captures the "strongest computational problem with codomain $\mathbb{N}$ that is Weihrauch reducible to $f$". This operator is very useful to prove separation results, especially at the higher levels of the Weihrauch lattice. We explore the first-order part in relation with several other operators already known in the literature. We also introduce a new operator, called unbounded finite parallelization, which plays an important role in characterizing the first-order part of parallelizable problems. We show how the obtained results can be used to explicitly characterize the first-order part of several known problems.

==> symbols.tex <==
\usepackage{ifthen}
\usepackage{xargs}

\usepackage{xcolor}

\makeatletter


\newcommand{\textdef}[1]{{\normalfont\textit{#1}}}

\renewcommand{\st}{{}\,:\,{}}

\def\function{\@ifstar\@function\@@function}
\newcommand{\@function}[2]{#1 \to #2}
\newcommand{\@@function}[2]{\colon #1 \to #2}

\def\mfunction{\@ifstar\@mfunction\@@mfunction}
\newcommand{\@mfunction}[2]{#1 \rightrightarrows #2}
\newcommand{\@@mfunction}[2]{\colon #1 \rightrightarrows #2}


\newcommand{\pfunction}[2]{:\subseteq #1 \to #2}
\newcommand{\pmfunction}[2]{:\subseteq #1 \rightrightarrows #2}

\newcommand{\charfun}[1]{\chi_{{#1}}}
\newcommand{\restrict}[1]{\ensuremath{\left. \hspace{-1mm} \right|_{#1}}}


\newcommand{\UTM}{\mathsf{U}}

\newcommand{\repmap}[1]{\delta_{#1}}


\newcommand{\str}[1]{({#1})}

\newcommand{\length}[1]{|{#1}|}
\newcommand{\concat}{\smash{\raisebox{.9ex}{\ensuremath\smallfrown} }}

\newcommand{\prefix}{\sqsubseteq}
\newcommand{\pprefix}{\sqsubset}
\newcommand{\extends}{\sqsupseteq}

\newcommand{\coding}[1]{\langle #1 \rangle}
\newcommand{\pairing}[1]{\langle #1 \rangle}


\newcommand{\seq}[1]{\mathbf{#1}}
\newcommand{\sequence}[2]{(#1)_{#2}}

\newcommand{\ran}{\operatorname{ran}}
\newcommand{\dom}{\operatorname{dom}}
\newcommand{\id}{\operatorname{id}}


\newcommand{\finStrings}[1]{{#1}^{<\mathbb{N}}}
\newcommand{\infStrings}[1]{{#1}^{\mathbb{N}}}

\newcommand{\Baire}{\mathbb{N}^\mathbb{N}}
\newcommand{\baire}{\finStrings{\mathbb{N}}}
\newcommand{\Cantor}{2^\mathbb{N}}
\newcommand{\cantor}{\finStrings{2}}

\newcommand{\turingreducible}{\le_{\mathrm{T}}}
\newcommand{\turingequiv}{\equiv_{\mathrm{T}}}
\newcommand{\turingincomparable}{~|_{\mathrm{T}~}}


\newcommand{\weireducible}{\le_{\mathrm{W}}}
\newcommand{\weistronger}{\ge_{\mathrm{W}}}
\newcommand{\weistrictlystronger}{>_{\mathrm{W}}}
\newcommand{\strictlyweireducible}{<_\mathrm{W}}
\newcommand{\weiequiv}{\equiv_{\mathrm{W}}}
\newcommand{\weiincomparable}{~|_{\mathrm{W}~}}


\newcommand{\strongweireducible}{\le_{\mathrm{sW}}}
\newcommand{\strictlystrongweireducible}{<_{\mathrm{sW}}}
\newcommand{\strongweiequiv}{\equiv_{\mathrm{sW}}}


\newcommand{\compproduct}{*}
\newcommand{\parallelization}[1]{\widehat{#1}}
\newcommand{\totalization}[1]{\mathsf{T}#1}
\newcommand{\completion}[1]{\ol{#1}}

\newcommand{\firstOrderPart}[1]{{}^1{#1}}
\newcommand{\ustar}[1]{#1^{u*}}


\newcommand{\lightfaceDelta}{\Delta}
\newcommand{\lightfaceSigma}{\Sigma}
\newcommand{\lightfacePi}{\Pi}
\newcommand{\lightfaceGamma}{\Gamma}
\newcommand{\boldfaceDelta}{\boldsymbol{\Delta}}
\newcommand{\boldfaceSigma}{\boldsymbol{\Sigma}}
\newcommand{\boldfacePi}{\boldsymbol{\Pi}}
\newcommand{\boldfaceGamma}{\boldsymbol{\Gamma}}



\newcommand{\Sier}{\mathbb{S}}

\newcommand{\LPO}{ \mathsf{LPO} }
\newcommand{\MLR}{\mathsf{MLR}}
\newcommand{\COH}{\mathsf{COH}}

\newcommand{\BWT}{ \mathsf{BWT} }


\newcommand{\RT}[2]{\mathsf{RT}^{{#1}}_{{#2}} }
\newcommand{\SRT}[2]{\mathsf{SRT}^{{#1}}_{{#2}} }
\newcommand{\cRT}[2]{\mathsf{cRT}^{{#1}}_{{#2}} }

\newcommand{\WWKL}{{ \mathsf{WWKL} }}
\newcommand{\WKL}{{ \mathsf{WKL} }}
\newcommand{\KL}{\mathsf{KL}}

\newcommand{\mflim}{\mathsf{lim}}

\newcommand{\PiBound}{\boldfacePi^1_1\mathsf{-Bound}}
\newcommand{\CodedBound}[1]{{#1}\mathsf{-Bound}}
\newcommand{\DS}{\mathsf{DS}}

\newcommand{\Choice}[1]{\mathsf{C}_{#1}}
\newcommand{\TChoice}[1]{\mathsf{TC}_{#1}}
\newcommand{\codedChoice}[3]{ {#1}\text{-}\mathsf{C}^{\vphantom{g}\mathsf{#2}}_{{#3}} }
\newcommand{\codedUChoice}[3]{\ifthenelse{\equal{#1}{}}{\mathsf{UC}^{\mathsf{\vphantom{g}#2}}_{{#3}} }{ {#1}\text{-}\mathsf{UC}^{\vphantom{g}\mathsf{#2}}_{{#3}} }}

\newcommand{\CNatural}{\mathsf{C}_{\mathbb{N}}}
\newcommand{\UCNatural}{\mathsf{UC}_{\mathbb{N}}}
\newcommand{\CCantor}{\mathsf{C}_{\Cantor}}
\newcommand{\UCCantor}{\mathsf{UC}_{\Cantor}}
\newcommand{\TCCantor}{\mathsf{TC}_{\Cantor}}
\newcommand{\CBaire}{\mathsf{C}_{\Baire}}
\newcommand{\UCBaire}{\mathsf{UC}_{\Baire}}
\newcommand{\TCBaire}{\mathsf{TC}_{\Baire}}

\newcommand{\chiPi}{\mathsf{WF}}
\newcommand{\PiCA}{\boldfacePi^1_1\mathsf{-CA}}

\newcommand{\SigmaWKL}{\boldfaceSigma^1_1\text{-}\mathsf{WKL}}
\newcommand{\SigmaCN}{\codedChoice{\boldfaceSigma^1_1}{}{\mathbb{N}}}
\newcommand{\SigmaCtwo}{\codedChoice{\boldfaceSigma^1_1}{}{2}}

\newcommand{\wfindHclosed}{\mathsf{wFindHS}_{\boldfacePi^0_1}}




\newcommand{\todo}[1]{{\color{red} #1}}


% added by Giovanni

\newcommand{\turreducible}{\le_{\mathrm{T}}}
\newcommand{\turstronger}{\ge_{\mathrm{T}}}
\newcommand{\turequiv}{\equiv_{\mathrm{T}}}
\newcommand{\strictlyturreducible}{<_\mathrm{T}}

\newcommand{\turdeg}[1]{{\bf #1}}

\newcommand{\Jump}{\mathsf{J}}

\newcommand{\Nb}{\mathbb{N}}

\newcommand{\ol}[1]{\overline{#1}}

\newcommand{\rst}{{\restriction}}

\newcommand{\rt}{\mathsf{RT}}
\newcommand{\srt}{\mathsf{SRT}}
\newcommand{\crt}{\mathsf{cRT}}
\newcommand{\csrt}{\mathsf{cSRT}}
\newcommand{\usrt}{\mathsf{u}\text{-}\mathsf{SRT}}

\newcommand{\tcn}{\mathsf{TC}_{\Nb}}
\newcommand{\lpo}{\mathsf{LPO}}
\newcommand{\isinf}{\mathsf{isInfinite}}
\newcommand{\isfin}{\mathsf{isFinite}}
\newcommand{\sort}{\mathsf{Sort}}
\newcommand{\isinfs}{\mathsf{isInfinite}_{\mathbb{S}}}
\newcommand{\isfins}{\mathsf{isFinite}_{\mathbb{S}}}

\makeatother

==> thref.tex <==
\makeatletter
\def\ifenv#1{
	\def\@tempa{#1}%
	\ifx\@tempa\@currenvir
	   \expandafter\@firstoftwo
	 \else
	   \expandafter\@secondoftwo
	\fi
}


\newcommand{\thlabel}[1]{%
	\label{#1}
	\begingroup
	\ifenv{theorem}{
		\def\@currentlabel{Theorem \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{unprovedtheorem}{
		\def\@currentlabel{Theorem \ref{#1}}
		\label{#1-th}
	}
 	{\ifenv{proposition}{
		\def\@currentlabel{Proposition \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{unprovedproposition}{
		\def\@currentlabel{Proposition \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{lemma}{
		\def\@currentlabel{Lemma \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{corollary}{
		\def\@currentlabel{Corollary \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{fact}{
		\def\@currentlabel{Fact \ref{#1}}
		\label{#1-th}
	}
	{\ifenv{definition}{
		\def\@currentlabel{Definition \ref{#1}}
		\label{#1-th}
	}
	{\GenericWarning{No Environment Found}}}}}}}}}
	\endgroup
}

\newcommand{\thref}[1]{\ref{#1-th}}

\makeatother
 
